Convexity Helps Iterated Search in 3D

Inspired by the classical fractional cascading technique, we introduce new techniques to speed up the following type of iterated search in 3D: The input is a graph $\mathbf{G}$ with bounded degree together with a set $H_v$ of 3D hyperplanes associated with every vertex of $v$ of $\mathbf{G}$. The goal is to store the input such that given a query point $q\in \mathbb{R}^3$ and a connected subgraph $\mathbf{H}\subset \mathbf{G}$, we can decide if $q$ is below or above the lower envelope of $H_v$ for every $v\in \mathbf{H}$. We show that using linear space, it is possible to answer queries in roughly $O(\log n + |\mathbf{H}|\sqrt{\log n})$ time which improves trivial bound of $O(|\mathbf{H}|\log n)$ obtained by using planar point location data structures. Our data structure can in fact answer more general queries (it combines with shallow cuttings) and it even works when $\mathbf{H}$ is given one vertex at a time. We show that this has a number of new applications and in particular, we give improved solutions to a set of natural data structure problems that up to our knowledge had not seen any improvements. We believe this is a very surprising result because obtaining similar results for the planar point location problem was known to be impossible.

==> app.tex <==
\section{Convex Overlays}\label{app:overlay}

\lemoverlay*

\begin{proof}
  Observe that the boundaries of each convex polytope is composed of vertcies,
  edges, and faces.
  Let $v$ be a vertex in the overlay $\A$.
  We have the following cases:
  \begin{enumerate}
    \item $v$ is a vertex in one of the original convex polytopes. 
      The number of vertcies of this type is clearly $O(n)$.
    \item $v$ is the result of the intersection an edge $e_i \in \P_i$ and $\P_j$ for
      $i\not = j$.
      Observe that each edge $e_i$ intersects each other convex polytope in at most two points.
      This means that each edge $e_i$ can create at most $m$ vertices of this type.
      Thus, the total number of vertices of this type is $O(nm)$.

    \item Finally, $v$ could be the result of the intersection of three faces $f_i \in \P_i$, $f_j \in \P_j$
      and $f_k \in \P_k$ for three distinct convex polytopes. 
      Observe that in this case, the $v$ is the result of the intersection of an edge $e_{ij}$ and the face $f_k$ where
      $e_{ij}$ is the intersection of the faces $f_i$ and $f_j$. 
      If we can prove that the number of such edges $e_{ij}$ is $O(mn)$, then the lemma follows by the same argument as the
      previous two.
      To prove this claim, observe that the edge $e_{ij}$ is also adjacent to two vertices which are the result of the intersection 
      of either $f_i$ and an edge of $\P_j$ or the intersection of an edge of $\P_i$ and $f_j$. In either case, by the previous arguments,
      the number of edges $e_{ij}$ is bounded by $O(mn)$. \qedhere
  \end{enumerate}
\end{proof}



\section{Proof of \reflem{basicpl}}\label{app:basicpl}

\basicpl*



\begin{proof}

    We decompose each $\P_i$ into its upper and lower hull, $U_i$ and $L_i$. 
    We can then turn each $U_i$ into a convex surface as follows: consider the projection of $U_i$ onto the
    $XY$-plane which will yield a convex 2D polygon $\P'_i$. Then, for every
    boundary edge $e$ of $\P'_i$, we
    add a hyperplane $h_e$ that goes through $e$. $h_e$ is made ``almost'' vertical (i.e., its angle with the 
    $XY$-plane is chosen close enough to $\frac{\pi}{2}$) such that the adding
    $h_e$ to the upper hull, for
    every boundary edge $e$, creates a convex surface $U'_i$ which can be represented as a function $\R^2 \rightarrow \R^3$
    (i.e., for every point $(x,y) \in \R^2$, there exists a unique value of $z$ such that $(x,y,z)  \in U'_i$).
    We repeat a similar process with the lower envelopes to create another surface $L'_i$.

    To build the data structure, we overlay all the surfaces in and let $\A$ be the resulting overlay. 
    By \reflem{overlay}, the complexity of the overlay $\A$ is $O(nm^2)$. 

    We decompose the overlay $\A$ into $O(m)$
    ``surfaces'', i.e., $Z$-monotone two-dimensional manifolds, as follows:
    Fix a value $i$. 
    Consider the set of points $q \in \R^3$ that have level $i$, i.e., $R_i= \left\{ q |\; |\Diamond(S,q^{\downarrow})| = i \right\}$.
    Define a surface $\S_i$ as the upper boundary of the closure of $R_i$. 
    Observe that $\S_i$ is a subset of the overlay $\A$ and it will also be a $Z$-monotone surface. 
    Recall that each surface $U'_j$ or $L'_j$ can be
    thought of as a function $\R^2 \rightarrow \R$, i.e., a function that is defined everyone on $\R^2$.
    It thus follows that the level of point
    $p$ can only change when lies on the intersection of two surfaces. 
    Thus, the process of creating layers does not create additional edges or vertices, meaning,
    in total the surfaces $\S_i$ have complexity $O(n m^2)$.

    Consequently, each surface $\S_j$ can be triangulated and also projected to the $XY$-plane
    and stored in a point location data structure.
    The triangles resulting from the triangulation are the triangles stored by the data structure. 

    Now consider queries.
    Given a query $q$, we can find the surface $\S_i$ that lies directly above $q$ using binary search on the at most $2m$ levels.
    Each step of the binary search can be done via a point location query for a total query time of $O(\log m \log n)$.
    This finds the triangle $\tau$ in the overlay $\A$ that lies directly above $q$.
    By construction, $\tau$ is the triangle claimed by the lemma.
\end{proof}

\section{Proof of~\reflem{int}}\label{app:int}

\lemint*

\begin{proof}

    \begin{figure}[h]
        \centering
        \includegraphics[scale=0.75]{figs/int}
        \caption{(1) An edge $e$ of $\Delta$ intersects  $\Delta'$.
            (2) A face $f'$ of $\Delta'$ intersects the boundary of $\Delta$ at a face $f$.
            (3) An edge of $\Delta'$ lies completely inside $\Delta$.  $e'$ is the intersection of
            two faces $f_1$ and $f_2$ of potentially two different polytopes. 
    }
        \label{fig:int}
    \end{figure}
   

  Consider a fixed cell $\Delta$ of $B$ and we count the number of cells $\Delta'$ that can intersect 
  $\Delta$.
  The cells $\Delta'$ and $\Delta$ can intersect at their boundaries
  or one could be contained in the other one. 
  We count the number of such cells $\Delta'$ using the following cases. 
  \begin{enumerate}
    \item An edge $e$ of $\Delta$  intersects $\Delta'$. Observe that every line can intersect each convex polytope
        in $A$ at most twice and thus $e$ can intersect $O(L)$ such cells. As $\Delta$ contains at most $\delta$ edges, 
        the number cells $\Delta'$ can be bounded by $O(L\delta)$.

    \item Now consider the case that a face $f'$  of $\Delta'$ intersects the boundary of $\Delta$, i.e. at a face $f$ of $\Delta$.
      Assume $f'$ lies on a face $F'$ of a polytope $\P'$ in $A$. 
      Let $s(F',f)$ be the line segment that is the intersection of the face $F'$ and the face $f$.
      We now consider two cases:
      (i) If $s(F',f)$ intersects the boundary of the face $f$ at an edge $e$ then it implies that an edge of $\Delta$ (the edge $e$) intersects
      $F'$. The number of such faces $F'$ is at most $O(L\delta)$ by the argument in the previous case and the segment $s(F',f)$ can also intersect at most
      $O(L)$ cells of $A$.
      Thus, the total number of cells $\Delta'$ that can fall in this case is $O(L^2 \delta)$ in total. 
      (ii) Now assume $s(F',f)$ does not intersect the boundary of $\Delta$ which implies it lies completely inside the face $f$ of $\Delta$, meaning,
      it has a vertex $v$ inside $f$.
      But in this case, $v$ is the result of the intersection of an edge of $\P'$ and $f$. 
      By assumptions, the number of such edges is at most $LX$, since there can be at most $X$ edges of every polytope $\P$ in $B$ intersecting $\Delta$. 
      As before, each of such edge can intersect $O(L)$ cells of $A$ and thus in total the number of cells $\Delta'$ that fall in this case
      is bounded by $O(L^2X)$. 
      Adding up the total from cases (i) and (ii) we get that the number of cells $\Delta'$ in this case is bounded by
      $O(L^2X + L^2 \delta)$.
      

    \item
        The first two cases cover the situation when the boundaries of $\Delta$ and $\Delta'$ intersect.
        We now consider when one cell contains the other.
        Observe that if $\Delta'$ contains $\Delta$, then $\Delta'$
        can be the only cell that intersects $\Delta$ and thus
        the only case left is when $\Delta'$ is fully contained in $\Delta$.
      In this case, consider one edge of $\Delta'$. 
      This edge will lie on the intersection of two faces $f_1$ and $f_2$ that could potentially belong to different polytopes in $A$. 
      Let $e'$ be the maximal line segment in which $f_1$ and $f_2$ intersect.

      First consider the sub-case when $e'$ intersects the boundary of $\Delta$ at a face $f$.
      This sub-case is very similar to the case 1:
      the face $f_1$  must intersect $f$, say at an edge $e_1$. If $e_1$ intersects an edge of $\Delta$, then it means that $f_1$ is one can be one of the $O(L\delta)$ faces intersected by
      the edges of $\Delta$ and thus the total number of edges $e_1$ that belong to this sub-case is $O(L\delta)$.
      Each such edge $e_1$ can intersect $O(L)$ faces as $f_2$, meaning, there are $O(L\delta^2)$ potential edges like $e'$ which in turn implies
      the total number of simplices $\Delta'$ that belong to this
      sub-case is $O(L\delta^3)$.

      The other sub-case is when $e'$ does not intersect the boundary of $\Delta$ which implies
      an end point $v$ of $e'$ lies  fully inside $\Delta$.
      Now, observe that the faces $f_1$ and $f_2$ are faces of two polytopes $\P_1$ and $\P_2$ and thus the 
      end points of the line segment $e'$ will be the result of the intersection of three faces of $\P_1$ and $\P_2$, meaning, two of the faces must come from
      the same polytope.
      W.l.o.g, assume that $v$ is the result of the intersection of $f_1, f'_1$ and $f_2$ where $f_1$ and $f'_1$ both belong
      to $\P_1$.
      Let $e_1$ be the boundary edge that lies between $f_1$ and $f'_1$. 
      Observe that $e_1$ must either cross the boundary of $\Delta$ or it must have a vertex (of the polytope $\P_1$) inside $\Delta$.
      In either case, we have a bound of $X$ for the number of such edges $e_1$ with respect to polytope $\P_1$ and 
      $O(XL)$ in total. 
      Each such edge $e_1$ can determine $O(L)$ other faces $f_2$ and each such intersection
      can in turn intersect $O(L)$ cells by the same argument.
      Thus the total in this case would be $O(XL^3)$. \qedhere
  \end{enumerate}
\end{proof}



%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> brief.tex <==




\begin{restatable}{theorem}{thmpath}\label{thm:path}
  If $\G$ is a path, then LEIS3D problem  can be solved with 
  a data structure that uses $O(n)$ space and with $O(\log n \LL n + |\bH|\log\log n)$ query time. 
\end{restatable}


\begin{restatable}{theorem}{thmgraph}\label{thm:graph}

    LEIS3D problem on a catalog graph $\G$ of maximum degree $d$ 
    can be solved with a data structure that uses $O(n)$ space and with 
    $O(\log n \LL n + |\bH|\sqrt{\log n \cdot \log d \cdot \log\log n})$ query time. 

\end{restatable}


Our main technical theorem is the following.

\frank{maybe remark that \bH does not have to be simple; i.e. it may
  revisit the same nodes, and cross etc.}


The above theorem leads to a number of applications. 
For example, one immediate application is the following.

\begin{restatable}{theorem}{thmthreedmax}\label{thm:3dmax}

    Let $P$ be a set of $n$ points in $\R^3$ each associated with a real-valued weight. 
    We can store $P$ in a data structure of $O(n\log n)$ size such that given a query
    halfspace $h$ one can find the point with maximum weight in $P \cap h$ in $\tilde{O}(\log^{3/2}n)$ time. 

\end{restatable}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> conc.tex <==
\section{Conclusions}


==> graph.tex <==
%\subsection{Catalog Graphs}
%Here, we show a simple application of our techniques that were developed
%in \refsec{tools} to show a non-trivial result on the LEIS problem for
%when the catalog graph $\G$ is an arbitrary graph of constant degree.
%
%
%\begin{restatable}{lemma}{lemgraph}\label{lem:graph}
%
%  Consider an instance of LEIS problem on a graph $\G$ of maximum degree $d$  and
%  let $n$ be the total input size. 
%  Given any parameter $\kappa < \log n$, we can build a data structure of size $\tO(n d^{O(\kappa)})$ 
%  such that for a LEIS query given by the pair $(q,\bH)$, we can
%  answer it in $O(\frac{|\bH|\log n\log\log n}{\kappa})$ time. 
%  The data structure can in fact solves the anchored version of the problem. 
%
%\end{restatable}
%
%\begin{proof}
%
%  Let $\Pi$ be the set of all walks of length $\kappa$ in $\G$.
%  As $\G$ has constant degree, we have $|\Pi| \le nd^{O(\kappa)}$.
%  For each path $\pi \in \Pi$, we build the data structure of \reflem{path}.
%  The total space consumption is $\tO(n 2^{O(\kappa)})$.
%
%  Now consider a query pair $(q,\bH)$.
%  Observe that we can divide $\bH$ into $O(\frac{|\bH|}{\kappa})$ walks of length
%  $\kappa$.
%  We query each path separately. 
%  Each query will require $O(\log n\log\log n)$ by \reflem{path} and thus the total query time is as claimed. 
%
%\end{proof}
%
%As before, using \reflem{2level} immediately improves the space complexity and we obtain the following theorem. 
%
%\thmgraph*
%
%\begin{proof}
%
%    We pick $\kappa = 2^{\sqrt{\log n\cdot \log^{-1}d\cdot \log\log n}}$ in \reflem{graph} and apply \reflem{2level}
%    with $\ell=d^{c\kappa} = 2^{c\log d\cdot \kappa}$ for a large enough constant $c$.
%    It is clear that the space consumption is  reduced to linear. 
%  Observe that by \reflem{2level}, we get that the query time is bounded by 
%  \[
%    O\left(\log n\log\log n + \frac{|\bH|\log n\log\log n}{\kappa} + |\bH|\log\ell\right)
%  \]
%  which is as claimed by the choice of our parameter $\kappa$.
%
%
%\end{proof}
%

\subsection{Weighted 3D Halfspace Range Searching}


\begin{theorem}
    We can give improved data structures for the following problems.
    \begin{itemize}
        \item (P1) weighted 3D halfspace range reporting: Let $P$ be a set of
        $n$ points in $\R^3$ such that each point $p_i$ is assigned
    a real-valued weight $w_i$.
    We would like to store the points in a data structure such that given a query halfspace $h$ and
    a range of weights $\zeta_1$ and $\zeta_2$, we can find all the points $p_i$ that are contained
    in $h$ and such that $\zeta_1 \le w_i \le \zeta_2$. 

    \peyman{Some ideas to think about later: given a set of $n$ weighted points in 2D, find  the closest 
    one with weight at least something or with weight in some range.}

    \end{itemize}
\end{theorem}


The following data structure is an immediate consequence of our  




==> path.tex <==
\subsection{Catalog Paths}

In this section, we will prove an almost optimal result on the LEIS problem for when the catalog graph $\G$ is a path.         


\begin{restatable}{lemma}{lempath}\label{lem:path}
  If $\G$ is a path of length $m$, then LEIS problem  can be solved with 
  a data structure that uses $O(n \log^3 (\LL n)^3)$ space and with $O(\log n \LL n + |\bH|)$ query time where
  $\bH\subset \G$ is the sub-graph given at the query time. 
  The data structure in fact solves the anchored version of the problem where the number of anchors is
  upper bounded by the claimed space complexity. 
\end{restatable}
\begin{proof}

    First observe that we can assume that length of the path path $\G$ is at most $t=\log n \LL n$:
    If the length of $\G$ is longer than $t$, we can simply
    break it into pieces of size $t$. 
    The number of pieces that will partially intersect the query subgraph $\bH
    \subset \G$ is at most two, meaning except for the two pieces, every other
    piece is either fully contained in $\bH$ or is completely disjoint from
    $\bH$.
    As a result, we can simply query each piece that intersects $\bH$ independently and separately. 
    Thus, in the rest of this proof, we will assume that $\G$ is a path of length at most $t$.

    To build the data structure, we  simply use \reflem{basicpl} which gives us a data structure
    with $O(n t^2)$ stored anchors.
    For each stored anchor, we store the list of polytopes that contain it resulting in a data structure
    with $O(n t^3)$ space. 

\end{proof}

As the above lemma solves the anchored version of LEIS, we can immediately apply 
\reflem{2level} with parameter $\ell=(\log n \LL n)^3$, and  obtain the following.

\thmpath*


==> removed.tex <==

    (ii) we let $x=\min\{ n, k 2^{C\sqrt{\log d\log n}}\}$ for a large enough
    constant $C$.
    Then, for each node $v \in \G$, we build a $x$-shallow cutting $C_v$ for the set of hyperplanes $H_v$.
    By \reflem{shallow}, $C_v$ can be assumed to be convex (i.e., the lower envelopes of some set of hyperplanes).
    The complexity of $C_v$ is also bounded by $O(\frac{|H_v|}{x})$.  
    Note that if $|H_v| < x$, then we will not store anything. In particular, in this case, the shallow cutting
    can be assumed to have only one cell with the entire set $H_v$ being its conflict list. 
    This implies that in total there are
    $r = O\left( \frac{n}{x} \right)$ hyperplanes in all the shallow cuttings,
    over all the vertices in $\G$.
    


  Let $A$ and $B$ be some small constants, and set parameters
  $m = A2^{B\sqrt{\log n}}$, and $\ell = \log_d m$. Similar to in
  \reflem{graphsc}, a vertex $v \in G$ is light if and only if their
  $x$-shallow cutting $C_v$ has size at most $d^{2\ell}$, and heavy
  otherwise.

  For each vertex $u$, we again consider all paths in \G of length
  $\ell$ starting at $u$, and organize them in a trie $\G_u$. If
  $\G_u$ contains heavy vertices, then we build a single
  \reflem{advpl} data structure on the $x$-shallow cuttings $C_v$,
  for all heavy vertices $v \in \G_u$. Observe that the number of
  input polytopes is at most $|\G_u| \leq d^\ell = m$, and that every
  polytope has complexity at least $d^{2\ell}$ since $v$ is heavy. Now
  since $\log^2(d^\ell/A) \leq d^{2\ell}$, we also have
  $m \leq 2^{\sqrt{\log d^{2\ell}}}$, and thus we can indeed apply
  \reflem{advpl}. Each anchor triangle $\tau$ in the
  \reflem{advpl} data structure stores a copy $\G_{u,\tau}$ of the
  trie $\G_u$. In turn, each node $v' \in \G_{u,\tau}$ again stores
  the at most three pointers to cells of $C_u$ containing the corners
  of $\tau$.

  Every vertex $u$ stores a trie $\G_u$ of size at most $m=d^\ell$,
  and a single \reflem{advpl} structure on $m$ convex polytopes. We
  again have that every vertex $v \in \G$ appears in at most
  $d^\ell=m$ such tries $\G_u$, and thus the total complexity of the
  convex polytopes that we use as input for the \reflem{advpl}
  structures is
  $O(\sum_{u \in \G} \sum_{v \in \G_u \land v \text{ is heavy}} |C_v|)
  = O((n/x)m)$. Thus the total space required for all these tries
  $\G_u$ and their \reflem{advpl} structures is bounded by $O((n/x)m)$
  as well. Each anchor triangle $\tau$ now stores a trie $\G_{u,\tau}$
  with $3m$ pointers. Therefore, by setting $x = \alpha km^2$ our data
  structure uses at most $O(n)$ space.

  Consider a query, consisting of a point $q \in \R^3$ and an initial
  vertex $u$ of the query subgraph $\H$. If $u$ is light, we simply
  directly query $C'_u$ in $O(\log m + \log(x/k))=O(\log m)$ time. If
  $u$ is heavy, we query the \reflem{advpl} data structure of
  vertex $u$, to get a anchor triangle $\tau$. We use the pointers
  associated with the copy $u'$ of $u$ in $\G_{u,\tau}$ to find the
  cells of $C_u$ containing the corners of $\tau$. For each corner, we
  query the secondary $k$-shallow cutting to report (pointers to the)
  at most three cells of the $k$-shallow cutting $C'_u$ containing
  $q$. This takes $O(\log (x/k))$ time. In both cases, we now get the
  next vertex $v$ of the query graph \bH, which is a neighbor of
  $u$. In case $v$ is light, we again directly query $C'_v$, but in
  case $v$ is heavy, we can instead move from node
  $u' \in \G_{u,\tau}$ to the node $v' \in \G_{u,\tau}$ corresponding
  to the copy of $v$. \frank{this is where we somehow need that the
    memory layout of the heavy nodes around $u'$ are stored in an
    identical way as the neighbors $v$ of $u$}. We can then use the
  pointers stored at $v'$ to once again find the prisms of $C_v$
  containing the corners of $\tau$. Finally, we then query the
  secondary $k$-shallow cutting of these three prisms with $q$,
  allowing us to answer the query for vertex $v$. We repeat this
  procedure for every next vertex of \bH. After $\ell$ steps, we may
  reach a heavy vertex $w$ that does not have a representative in
  $G_{u,\tau}$, in which case we query the \reflem{advpl} data
  structure of vertex $w$, and continue the query in the same way as
  described above.

  In total, we spend $O(\bH\log m)$ time to answer the light
  queries. The total time spend on the queries to the \reflem{advpl}
  data structure is
  $O(\lceil \frac{|\bH|}{\ell} \rceil\log n\LL^c n)$. \frank{TODO;
    fill in the $c$}.  Finally, the time for all queries to the
  secondary $k$-shallow cuttings is
  $O(|\bH|\log (x/k)) = O(|\bH|\log m)$. Hence, our total query time
  is again
  $O(|\bH|\log m + \lceil \frac{|\bH|}{\ell} \rceil\log n\LL^c
  n)$. So, plugging in $m = A2^{B\sqrt{\log n}}$ gives us a query time
  of $O(\log n\LL^c n + |\bH|\sqrt{\log n})$ as claimed.

\subsection{The Basic Technique}

Our main result here is a data structure that can solve our problem (but not the on-demand version).
We will later present a solution for the on-demand variant but we believe there
is value in also independently presenting our simpler solution here. 


\begin{restatable}{lemma}{lembasic}\label{lem:basic}
    LEISD3D problem can be solved with a data
    structure that uses $O(n)$ space and with the query time of 
    (i) $O(\log n \log\log n + |\bH|\log\log n)$ for when $\G$ is a path or 
    (ii) $\overline{O}(\log n  + |\bH|\sqrt{\log n \log d})$ for when $\G$ is a graph of maximum degree $d$.

\end{restatable}

\frank{if $k \approx n$ then $x$ exceeds $n$. Say s.t. about that case.}

\begin{proof}

    First observe that regarding case (i), we can assume that length of the path  $\G$ is at most $t=\log n \LL n$:
    If the length of $\G$ is longer than $t$, we can simply
    break it into pieces of size $t$. 
    The number of pieces that will partially intersect the query subgraph $\bH
    \subset \G$ is at most two, meaning except for the two pieces, every other
    piece is either fully contained in $\bH$ or is completely disjoint from
    $\bH$.
    As a result, we can simply query each piece that intersects $\bH$ independently and separately.

    We now describe the data structure.
    Let $x$ be a parameter that depends on the graph $\G$:
    in case (i) we let $x=\min\{n,k( \log n \log\log n)^3\}$ and in case (ii) we let $x=\min\{ n, k 2^{C\sqrt{\log d\log n}}\}$ for a large enough constant $C$.
    Then, for each node $v \in \G$, we build a $x$-shallow cutting $C_v$ for the set of hyperplanes $H_v$.
    By \reflem{shallow}, $C_v$ can be assumed to be convex (i.e., the lower envelopes of some set of hyperplanes).
    The complexity of $C_v$ is also bounded by $O(\frac{|H_v|}{x})$.  
    Note that if $|H_v| < x$, then we will not store anything. In particular, in this case, the shallow cutting
    can be assumed to have only one cell with the entire set $H_v$ being its conflict list. 
    This implies that in total there are
    $r = O\left( \frac{n}{x} \right)$ hyperplanes in all the shallow cuttings,
    over all the vertices in $\G$.
    
    In addition, for every triangle $\tau$ in the shallow cutting $C_v$, we compute the conflist
    list, $L_\tau = \Diamond(H_v,\tau^{\downarrow})$, and then we build a $k$-shallow cutting on $L_\tau$;
    we call these shallow cuttings, over all triangles $\tau$ in $C_v$,  
    \textit{the secondary shallow cuttings}.


    To build the data structure, we will use \reflem{basicpl}, however, slightly differently whether we are in 
    case (i) or (ii). In the former case, we use it on all the shallow cuttings $C_v$, for all $v \in \G$ and in
    the latter case, we use it on every path of length $\ell = \sqrt{\frac{\log n}{\log d}}$ in the graph $\G$
    (meaning, for every path $\pi$ of length $\ell$, we use it on the shallow cuttings $C_v$ for all
    the vertices $v \in \pi$). 
    In case (i), this gives us a data structure with $O(r t^2)$ stored anchors.
    In case (ii), observe that each node of $\G$ appears in at most $d^\ell = d^{\sqrt{\frac{\log n}{\log d}}} = 2^{\sqrt{\log d \log n}}$ 
    paths and on each path, we are
    overlaying fewer than $\sqrt{\log n}$ convex polytopes 
    and thus the total number of anchors is bounded  by $O(r \log n
    2^{\sqrt{\log d\log n}})$.


    
    In either case, consider one anchor $\tau$
    and let $A_1, A_2$, and $A_3$ be the vertices of
    $\tau$.\frank{weird names for points $p_1,,p_3$?}
    \peyman{I think sometimes we use $p_i$ for input points. We also have $v$ for vertices of $\G$}
    Then consider each vertex $v \in \G$ that was used to build the overlay where $\tau$ belongs to. 
    If $\tau$ is not below the $x$-shallow cutting $C_v$, then we simply store this information at $\tau$.
    Otherwise, for each $A_i$, $1 \le i \le 3$, let $\psi_{i,v}$ be
    the prism in $C_v$ that contains $A_i$.
    We place a pointer from $\tau$ to $\psi_{i,v}$, for $1 \le i \le 3$.
    This concludes the our preprocessing.

    Observe that 
    the number of pointers placed from an anchor in case (i) is at most $\log n \LL n$ and in case (ii) it is
    at most $\ell < \sqrt{\log n}$. 
    By the choice of $r$, it follows that our space consumption is linear. 

    We now explain the query process.
    In case (i), we simply have to answer the query on the entire path $\G$ of length at most $\log n \LL n$.
    In case (ii), we can reduce the problem to answering the query on
    paths of length at most $\ell$. For example by computing a
    spanning tree of $\H$, constructing an Euler tour of this tree,
    and splitting this tour into $O(\frac{|\H|}{\ell})$ paths of length at
    most $\ell$.
    In either case, we have implemented an instance of \reflem{basicpl} on a (relevant) path $\pi$ and thus we can obtain 
    an anchor $\tau$ as the result of the query.
    In the preprocessing time, for each node $v \in \pi$, and each anchor $\tau$, we have noted whether $\tau$ is below or
    above $x$-shallow cutting $C_v$.
    If it is above, then there is nothing to for node $v$ and we can simply return that the query point is above the $k$-level
    of $H_v$ as $x \ge k$. 
    Thus consider the latter case in which we can locate the three prisms $\psi_{i,v}$, for $1 \le i \le 3$ via pointers
    stored at $\tau$. 
    By \refob{below}, $\Diamond(H_v,\tau^{\downarrow}) \subset \cup_{i=1}^3 \Diamond(H_v,A_i^{\downarrow})$
    and also observe that as $q$ is below $\tau$, we have $\Diamond(H_v,q^{\downarrow})\subset \Diamond(H_v,\tau^{\downarrow})$.
    As a result, we simply query the point location data structure built on the secondary $k$-shallow cuttings stored
    for each $\psi_{i,v}$. 
    If for any of them, it turns out that $q$ lies above the $k$-level, then it also lies above the $k$-level of $H_v$ and thus
    we are done.
    \frank{We even have $x \geq \alpha k$, and thus the point lies
      actually above our $k$-shallow cutting. I could imagine
      applications where we actually want that.}
    
    Otherwise, we can find three cells $\Delta_1, \Delta_2$ and $\Delta_3$ in the secondary shallow cuttings of
    $\psi_{1,v},\psi_{2,v}, \psi_{3,v}$ respectively.
    We return (pointers to) the conflict lists of these three cells as
    the answer to our query.
    % The conflict list of these cells (in the secondary shallow cutting) is the pointers returned by the query.
    Based on the above observation, the correctness of the query algorithm is guaranteed.

    It remains to analyze the query time.
    In case (i), the query time is the direct consequence of \reflem{basicpl}. 
    In case (ii), we can subdivide $\bH$ into $O(\frac{|\bH|}{\ell})$
    paths of length $\ell$ in $O(|\bH|)$ time.
    In each path, the use of \reflem{basicpl} requries $\overline{O}(\log
    n)$ time to locate the anchor $\tau$.
    \frank{actually: it is not so clear how we find the
      \reflem{basicpl} structure corresponding to this path. (o)
    }
    However, on every vertex of $v \in \bH$, we also do three point location queries on the secondary shallow cuttings. 
    However, observe that each point location requires $O(\log(x/k)) = O(\sqrt{\log d \log n})$ query time.
    Thus, the total query time will be $\overline{O}(\frac{|\bH|}{\ell}\log n  + |\bH| \sqrt{\log d \log n})$ which is
    as claimed. 
\end{proof}


\paragraph{Remark.}
Our data structure works in the real RAM model but it is also possible to make it work in variants of the
pointer machine model.
We will discuss these issues in the appendix. 

%The sticking point is finding the correct data structure of \reflem{basicpl}.
%In particular, assume that a query subgraph $\bH \subset \G$ is given and we have divided into paths of
%length $\ell$. For every vertex $v \in \G$, we have an instance of the data structure of \reflem{basicpl}.


\subsubsection{Fixing the space issue and the pointer machine stuff}
\label{ssub:Fixing_the_space_issue}

\frank{new attempt}
\frank{assume that $k \geq 1$ for simplicity of the writeup;}

Let \G be our input graph, in which each vertex $v$ is associated with
a set $H_v$ of planes, and let $k \in 0..n$ be a parameter. For ease
of description we will assume that $k \geq 1$ in the remainder of this
section.

Our main result here is a data structure that can solve the shallow
cutting version of our problem (but not the on-demand version).  We
will later generalize this solution but we believe there is value in
also independently presenting it because the solution is much simpler.

Let $\ell$ and $x$, with $x \geq \alpha k$, be two parameters whose
exact value we specify later. For each vertex $u$ in our input graph
\G, we will construct an $x$-shallow cutting\footnote{When $x > |H_u|$
  we define $C_u$ to consist of a single ``prism'' which is just
  $\R^3$. With some abuse of notation we will still refer to $C_u$ as
  an $x$-shallow cutting.} $C_u$ of the planes in $H_u$. This cutting
has size $O(|H_u|/x)$, and each prism has a conflict list of size
$O(x)$. We will store (the vertical projection of) $C_u$ in a planar
point location structure so that given a query point $q \in \R^3$, we
can find the prism of $C_u$ containing $q$ in $O(\log (n/x))$ time. We
will refine $C_u$ into the desired $k$-shallow cutting $C'_u$;
i.e. for each prism $\Delta$ in $C_u$, we construct a $k$-shallow
cutting $C'_{u\Delta}$ of size $O(x/k)$ on its conflict list and clip
the result to $\Delta$. We again process these \emph{secondary}
shallow cuttings $C'_{u\Delta}$ for efficient point location queries,
and compute their conflict lists. The union of these secondary
cuttings $C_{u\Delta}$, over all prisms $\Delta \in C_u$, defines the
$k$-shallow cutting $C'_u$ associated with $u$. The total space used
for vertex $u$ is $O(|H_u|)$, and thus $O(n)$ in total.

\frank{below is a weird mix of details still}

Our main idea is now to cover $\G$ with paths of length $\ell$, and
build \reflem{basicpl} data structures on the $x$-shallow cuttings
$C_v$ for all nodes $v$ in the path. These \reflem{basicpl} data
structures store sets of anchor triangles. For each such an anchor
triangle $\tau$ we store a copy of the path $P$, with, for each node
$v$ three pointers: for every corner $p_i$ of $\tau$ we store the cell
$\Delta_{v,i}$ of $C_v$ containing $p_i$ (if it exists). This will
allow us to efficiently find these cells $\Delta_{v,i}$, for every
vertex $v \in \bH$. 

%\thmpath*
path theorem.

\begin{proof}
  Set $\ell = \log n\LL n$. We say a vertex $u \in \G$ is \emph{light}
  if $C_u$ has size at most $\ell^3$, and \emph{heavy} otherwise.

  For each vertex $u \in \G$, consider the path $\G_u$ in \G of length
  $\ell$ starting at $u$. We store the $x$-shallow cuttings $C_v$ of
  all heavy vertices $v \in \G_u$ (if there are any) in a
  \reflem{basicpl} data structure. For each anchor triangle $\tau$
  stored by this data structure, we store a copy $\G_{u,\tau}$ of the
  path $\G_u$. For each node $v' \in \G_{u,\tau}$ we store (at most)
  three pointers: for each corner $p_i$ of $\tau$ we store the pointer
  to the prisms of $C_v$ containing $p_i$ if such a prism exists.

  Each \reflem{basicpl} data structure uses
  $O(\sum_{v \in \G_u \land v \text{ is heavy}}|C_v|\ell^2)$ space,
  and stores the same number of anchor triangles. In turn, each such
  an anchor triangle stores a copy of $\G_u$, which has size
  $O(\ell)$. Hence, the total space used for $\G_u$ is
  $O(\sum_{v \in \G_u \land v \text{ is heavy}}|C_v|\ell^3)$. Each
  heavy vertex $v$ appears in at most $\ell$ paths $\G_u$, and $C_v$
  has size $O(|H_v|/x)$. So, summing over all paths $\G_u$ we obtain
  $O(\sum_{u \in \G} \sum_{v \in \G_u \land v \text{ is
      heavy}}|C_v|\ell^3) = O(\sum_{v \in \G \land v \text{ is
      heavy}}|C_v|\ell^3) = O(\ell^3(n/x))$. By setting
  $x=\alpha k\ell^3$ (where $\alpha$ is the universal constant from
  \reflem{shallow}) we can now make sure our \reflem{basicpl} data
  structures use a total of $O(n/k)$ space. Hence, the total space
  used by our data structure is $O(n)$ (since we also need to store
  all $k$-shallow cuttings and their conflict lists).

  To answer a query $q,\bH$, we do the following. If a vertex
  $u \in \bH$ is light, we directly query the $k$-shallow cutting
  $C'_u$ of vertex $u$. More specifically, we query $C_u$ to find the
  cell $\Delta$ containing $q$ (if it exists), and then and then query
  its secondary cutting $C'_{u,\Delta}$ to find at most one cell
  containing $q$. This takes $O(\log (\ell^3) + \log(x/k))$ time, and
  thus $O(|\bH|\log (\ell^3) + \log(x/k))$ time in total.

  If a vertex $u \in \bH$ is heavy, we query its \reflem{basicpl} data
  structure with $q$, giving us a triangle $\tau$ above $q$. We then
  follow the query path $\bH$ in the copy $\G_{u,\tau}$ of $\tau$. For
  each node $v' \in \G_{u,\tau}$, which is some copy of a node
  $v \in G$, we follow the pointers stored at $v'$ to locate the
  prisms $\Delta_1,\Delta_2,\Delta_3 \in C_v$ containing the corners
  of $\tau$. \reflem{basicpl} guarantees that $q$ lies in the convex
  polytype corresponding to $C_v$ if and only if $\tau$ is contained
  in $C_v$. So If a corner of $\tau$ lies above $C_v$; then $q$ also
  lies outside of $C_v$. Since $x \geq \alpha k$, it means $q$ also
  lies above the $k$-shallow cutting $C'_v$. If the three prisms
  $\Delta_1,\Delta_2,\Delta_3$ all three exist, we query their
  secondary $k$-shallow cuttings with $q$, and report the at most
  three prisms $\Delta'_1,..,\Delta'_3$ of $C'_v$ we find. By
  \reflem{ob:below} the set of planes from $H_v$ below $q$ is a subset
  of these three conflist lists.

  The above query procedure thus allows us to answer the query for all
  $\ell'$ heavy vertices on the subpath $\G_u$ of length $\ell$, in at
  most $O(\ell + \ell' \log(x/k))$ time (the cost to locate $q$ in the
  secondary shallow cuttings). Hence, the total number of queries to
  the \reflem{basicpl} data structure that we need is at most
  $O(\lceil \frac{|\bH|}{\ell} \rceil)$, and the time spend on these
  queries is $O((\lceil \frac{|\bH|}{\ell} \rceil \log n\log
  \ell)$. It follows that the total time spent on all heavy vertices
  is
  $O((\lceil \frac{|\bH|}{\ell} \rceil \log n\log \ell +
  |\bH|\log(x/k))$. The total query time is thus
  $O(\lceil \frac{|\bH|}{\ell} \rceil\log n\log \ell + |\bH|\log(x/k)
  + |\bH|\log \ell) = O(\log n\LL n + |\bH|\LL n)$.
\end{proof}

Next, we consider the case that $\G$ is an arbitrary graph whose
vertices have degree at most $d$, and the query graph \bH is given at
once at query time. The main difference is that we will now construct
multiple \reflem{basicpl} data structures for \emph{every} vertex
$u \in \G$; in particular, one for every path of length $\ell$
starting at $u$. As a result, we choose our parameters slightly
differently.

graph theoreym
%\thmgraph*
\frank{the leading term is not quite right yet. it seems it should
  have a $d$ somewhere.}

\begin{proof}
  Set $\ell = \sqrt{\frac{\log n}{\log d}}$. We now say a vertex
  $u \in \G$ is \emph{light} if $C_u$ has size at most
  $\ell^3 d^\ell$, and $\emph{heavy}$ otherwise.

  For each vertex $u$, now consider all paths in \G of length at most
  $\ell$ that start at $u$. We organize these paths in a trie
  $\G_u$. If (and only if) $\G_u$ contains any heavy vertices $v$,
  then we store $\G_u$. Consider the path $P_w$ in $\G_u$ from $u$ to
  some vertex $w$. We store a \reflem{basicpl} data structure on all
  $x$-shallow cuttings $C_v$ for all heavy nodes on $P_w$. For each
  anchor triangle $\tau$ in this data structure, we again store a copy
  $P_{w,\tau}$ of path $P_w$, with for each vertex $v' \in P_w$
  pointers to the cells of $C_v$ containing the corners of $\tau$ as
  in \reflem{lem:path}.

  There are at most $O(d^\ell)$ paths of length at most $\ell$ that
  start at $u$. Hence, each (non-empty) trie $\G_u$ has size at most
  $O(d^\ell)$. Symmetrically, a heavy vertex $v$ appears in the trie
  $\G_u$ of at most $O(d^\ell)$ other vertices $u$. Each node in
  $\G_u$ stores a \reflem{basicpl} data structure on at most $\ell$
  shallow cuttings $C_v$. Since for each heavy vertex $v$, $C_v$ also
  appears in $O(d^\ell)$ tries $\G_u$, the overall size of all these
  \reflem{basicpl} data structures is thus
  $O\left(\sum_{u \in \G} \sum_{v \in \G_u \land v \text{ is heavy}}
    |C_v|\ell^2\right) = O((n/x)d^\ell\ell^2)$. Each anchor triangle
  stores a list of $3\ell$ pointers. Hence, setting
  $x = \alpha kd^\ell\ell^3$ it follows that this is at most
  $O(n/k)$. The total space usage of our structure is thus again
  $O(n)$.

  We can now answer a query $q, \bH$. Observe that in $O(|\bH|)$ time,
  we can transform \bH into a path of length $O(|\bH|)$, i.e. by
  computing an Euler tour of a spanning tree of \bH. Hence, in the
  remainder we assume \bH is path. For all light vertices $v$ of \bH,
  we simply query $C'_v$ with point $q$ directly. This takes
  $O(|\bH|\log (\ell^3 d^\ell))$ time in total. To obtain the answers
  for the heavy vertices we query the \reflem{basicpl} data
  structures. In particular, for the first heavy vertex $u$ on $\bH$,
  we follow the path in $\G_u$ corresponding to the next $\ell$
  vertices on $\bH$. We query the \reflem{basicpl} data structure
  associated with this path $P$, which gives us a triangle $\tau$
  directly above $q$. For each of the vertices $v$ of $P$, we can now
  again follow the pointers to the three prisms of $C_v$ containing
  the corners of $\tau$, and query the secondary $k$-shallow cuttings
  of these cells with $q$. In total, we make
  $O(\lceil \frac{|\bH|}{\ell} \rceil)$ queries to \reflem{basicpl}
  data structures, taking
  $O(\lceil \frac{|\bH|}{\ell} \rceil \log n\log \ell)$ time in
  total. The point location queries in the secondary $k$-shallow
  cuttings take a total of $O(|\bH|\log(x/k))$ time. Putting all of
  this together, the query time is
  $O(|\bH|\log(\ell^3d^\ell) + \lceil \frac{\bH}{\ell} \rceil\log
  n\log \ell + |\bH|\log(x/k)) = O(|\bH|\log(\ell^3d^\ell) +
  \lceil\frac{\bH}{\ell}\rceil \log n\log \ell) = O(\log n\LL n +
  \bH\sqrt{\log n\log d})$.
\end{proof}
\frank{we should pick $\ell$ slightly differently it seems?}


\subparagraph{On demand $\bH$.} Finally, we extend the above result to
the case \bH is a path that is given on-demand. The main difference is
that, for a given heavy vertex $u$, we do not know which path in
$\G_u$ to explore. Hence, we do not know which \reflem{basicpl} data
structure to query. So instead, we will build a point location data
structure on \emph{all} (heavy) vertices in $\G_u$ at once. However,
with the \reflem{basicpl} data structure, this means such a query
would take $O(\log n \log (d^\ell)) \approx O(\log n\ell)$ time. Since
we need $O(\bH/\ell)$ such queries, we end up with a query time of
$O(\bH\log n)$. Hence, we may as well query every $k$-shallow cutting
$C'_v$ separately. So, instead, of the \reflem{basicpl} data
structure, we use the \reflem{advanced} data structure instead.



